SIMD$^2$: A Generalized Matrix Instruction Set for Accelerating Tensor Computation beyond GEMM

Matrix-multiplication units (MXUs) are now prevalent in every computing platform. The key attribute that makes MXUs so successful is the semiring structure, which allows tiling for both parallelism and data reuse. Nonetheless, matrix-multiplication is not the only algorithm with such attributes. We find that many algorithms share the same structure and differ in only the core operation; for example, using add-minimum instead of multiply-add. Algorithms with a semiring-like structure therefore have potential to be accelerated by a general-purpose matrix operation architecture, instead of common MXUs. In this paper, we propose SIMD$^2$, a new programming paradigm to support generalized matrix operations with a semiring-like structure. SIMD$^2$ instructions accelerate eight more types of matrix operations, in addition to matrix multiplications. Since SIMD$^2$ instructions resemble a matrix-multiplication instruction, we are able to build SIMD$^2$ architecture on top of any MXU architecture with minimal modifications. We developed a framework that emulates and validates SIMD$^2$ using NVIDIA GPUs with Tensor Cores. Across 8 applications, SIMD2 provides up to 38.59$\times$ speedup and more than 10.63$\times$ on average over optimized CUDA programs, with only 5% of full-chip area overhead.

==> Makefile <==
MY_DATE := $(strip $(shell date +"%F_%H_%M_%S"))

ifeq ($(OS),Windows_NT)
$(warning Windows NT detected "$(USER)")
DVI = yap
DVIBIN = yap
DISTILL = "$(HOME)"/bin/acrodist.exe

PREFIX=c:\\cygwin\\home\\$(USER)\\papers\\2008SASP-arsenal\\
ACROREAD = "$(HOME)"/bin/acroread.exe
ALL = show_nt
else # mac

ifeq ($(USER),mbt)
ALL = show_nt
ACROREAD = mupdf-x11
else
ALL =  pdf
endif

endif

TEX_STUFF= $(wildcard *.tex)
PDF_TARGETS= paper.pdf 
#extended-abstract.pdf
#paper_revision.pdf
FIGURES = $(wildcard Figures/*.pdf) $(wildcard Graphs/*.pdf)

.PHONY: test_build clean

all: $(ALL)

paper.pdf:  $(FIGURES) Makefile 

figs:
	make -C Figures


test_build:
	rm -rf _test_build
	mkdir _test_build
	(REPO=$$(svn info | grep URL | sed 's/URL: //');\
	 DIR=$$(svn info | grep URL | sed 's/.*\///');\
	 cd _test_build; \
	 svn checkout $$REPO;\
	 cd $$DIR;\
	 make;\
	 open paper.pdf;\
	)	

%_abbrv.bib: %.bib
	./abbrv.py $< $@

pdf: $(PDF_TARGETS)

%.aux : %.tex $(TEX_STUFF)
	pdflatex $(PDFLATEX_BATCH_OPTIONS) $* 

%.bbl : %.aux 
	bibtex $* || true

%.pdf : %.bbl figs
	pdflatex $(PDFLATEX_BATCH_OPTIONS) $*
	pdflatex $(PDFLATEX_BATCH_OPTIONS) $*
	killall -s1 mupdf-x11 2>/dev/null
	pdftops $*.pdf
	ps2pdf14 -dPDFSETTINGS=/prepress $*.ps
#	cp $*.pdf 122-OX997-Tseng.pdf
#
# copies file to prevent write-after-read problems
# uses date as suffix.
#
show_nt: pdf
	- killall $(ACROREAD)
	cp paper.pdf paper_$(MY_DATE).pdf
	$(ACROREAD) $(PREFIX)paper_$(MY_DATE).pdf &

clean:
	rm -rf *.aux *.log *.bbl *.blg *.out *.ps $(PDF_TARGETS)
	rm -rf paper_abbrv.bib 
	rm -rf _test_build
	make -C Figures/ clean





==> background.tex <==
\section{Background and Motivation}
\label{sec:mxu}

Though matrix semirings can easily express matrix algorithms, conventional
architectures do not efficiently support this paradigm. 

We first cover background in MXUs and matrix algorithms 

\subsection{Background: Conventional MXU abstractions}
MXU performs matrix-matrix operations to reduce data movement.
An MXU performs a tile of a larger matrix operations.
Define what is an MXU operation in algorithm (forloop) forms
Then claim that different MXU are just different scale of this form
(e.g., tensor core is 8x8x8, TPU MXU is 128x128x128)

MXU is everywhere.

Make another point about MXU can be broken down in to data feeding part and operation part.
This allows us to say data feeding part (tiling) is complicated, but operation part (MAC) is simple.
Nonetheless, but changing the operation part, we can now support many more matrix algorithms natively, as shown in later section.

data input format style and dataflow

Workflow == operation == \CMO{}




\subsection{Motivation: General matrix algorithms with \CMO{}}

Many applications have the form of transitive closure or \CMO{}

Transformation has been found in the 70s and 80s.

With MXU available, transformation enables easy hardware acceleration 

Have the formal definition(s) matrix algorithms here.
Talk about GEMM is one instance of the such algorithms.
Show case one algorithm that share the same form but just different \CMO{}
again in the algorithm (forloop) form.

Talk about how many possible operations are there and we explore two in this paper

%\input{applications}

\subsection{Contribution}
We connect the high-level idea in transformation
and our knowledge in MXU to design and propose general purpose MXU.
If other people have done it, they will end up with multiple sets of individual accelerators.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{
\section{Background}
\label{sec:background}
\cfigure[Figures/conventionalStore.pdf,{The blocked-matrix-multiplication datapath in a hardware-accelerated computing system having a conventional storage-system hierarchy with non-volatile memory (NVM)},fig:conventionalStore]
The dimensionality mismatch among hardware accelerators, memory devices, and abstractions is a primary source of processing inefficiency. This section explains the effects of mismatching dimensionalities on application performance, the challenges of tackling such mismatches, and the limitations of current research attempting to address the problem.
%paths that attempt to address the problem.

\subsection{Modern accelerator-based architectures}
\label{sec:conventional_model}

Figure~\ref{fig:conventionalStore} shows the key hardware components for processing high-dimensional datasets in a modern heterogeneous computer. Such a computer typically uses hardware accelerators (e.g., GPUs in Figure~\ref{fig:conventionalStore}) to perform compute kernels on high-dimensional datasets. Modern GPUs provide two types of processing elements: (1) conventional GPU cores that operate on vectors and (2) TCUs that operate on matrices to more efficiently process high-dimensional datasets. %\CMFcom{As intended?}.

To provide high-performance data storage, a computer may use a solid-state drive (SSD) that stores data in non-volatile memory technologies such as NAND flash memory and phase-change memory (PCM). All non-volatile memory technologies have their own basic access granularities (e.g., page in flash memory). This is true for newer byte-addressable devices like PCM~\cite{WuUnwrittenContract3DXPoint}. To improve bandwidth, modern SSD controllers use channel-level and bank-level parallelism. Modern SSDs typically organize their memory arrays into channels, with all parallel channels capable of accepting unique requests simultaneously. Each channel also contains multiple banks that allow free banks to accept requests while other banks are busy. Commercialized non-volatile memory technologies have limited program-erase cycles, so SSD controllers must carefully manage mapping between the logical addresses that software uses and physical addresses in memory.

Because modern storage systems still expose linear address spaces such as logical block addresses (LBAs) for use, producers of high-dimensional datasets must reduce data dimensionality to 1-dimensional representations, typically with row-oriented or column-oriented storage formats. If a hardware-accelerated compute kernel needs to compute on datasets, an application invoking the compute kernel must first fetch each piece of necessary data from the storage system. The application then assembles each received data chunk into memory objects with a layout that satisfies the demands of the target accelerator’s architecture. Finally, the application copies the created memory object from the host main memory to the accelerator’s device memory so compute kernels can use the object.


Figure~\ref{fig:conventionalStore} also shows matrix multiplication (MM) performed using a modern GPU. The GPU kernel delivers maximum computation throughput if the MM kernel is performed on 8K\x{}8K submatrices. The origin dataset presents its matrix inputs using a row-oriented storage format, which is generally considered the most efficient for CPU-based compute kernels. Each raw input matrix is 16K\x{}16K. The SSD has 8KB pages and 8 parallel channels; each SSD page stores 2K elements encoded in IEEE-754 32-bit floating-point format, and each matrix row occupies 8 pages that are logically consecutive in the SSD’s LBA. In conventional SSD design, these consecutive pages are typically striped across different channels to enable sequential parallel accesses in LBAs; such striping is needed because most file systems and applications assume
%are designed with the assumption 
that underlying storage devices are more efficient when the devices perform accesses sequentially. As a result, each of the aforementioned 8 pages that belongs to a single row will be physically located in a distinct channel.

To maximize the efficiency on machines that have only limited high-speed memory capacity available for hardware accelerators, an application must create a pipeline to logically partition input matrices into submatrices and perform multiplications on pairs of submatrices. In each pipeline, the application first creates a submatrix by retrieving necessary elements from all required rows into a destination location in system main memory. Once all elements of a submatrix have arrived, the application copies the created submatrix to the accelerator’s device memory and launches the compute kernel on the copied submatrix.

%\cfigure[Figures/CPUOverhead.pdf,{The relative execution time of matrix multiplications using row-store format (sequential) and sub-block format, with data already in main memory.},fig:cpu_overhead]

\dcfigureSingleCol[Figures/CPUOverhead.pdf,Figures/SSDOverhead.pdf,{The relative execution time of matrix multiplications using row-store format (sequential) and sub-block format, with (a) data already in main memory and (b) from the SSD.},fig:cpu_overhead]

\noindent\textbf{[P1]: The overhead of marshalling input data.} 
To restructure stored data into the dimensionality hardware accelerators need, an application must use CPU instructions to calculate the mapping between the raw-data offset and the target memory locations. Then the application must issue I/O requests through the system software stack, again using CPU instructions, to fetch pieces of raw data and place (and potentially convert) the received data chunks in their designated memory locations. In Figure~\ref{fig:conventionalStore}, if the application needs to fetch an 8K\x{}8K submatrix, the row-store format will require the program to issue 8,192 I/O requests---to fetch 8,192 rows that contain the submatrix items.

Figure~\ref{fig:cpu_overhead}(a) illustrates the CPU overhead, with the raw data already in system main memory before the compute kernel launches. The system uses an AMD RyZen 3700X CPU and Nvidia’s RTX 2080 GPU. The baseline comprises pipelined matrix multiplications---that is, the multiplication of two 32K\x{}32K matrices using sub-blocks of 8K\x{}8K matrices. As the source dataset uses sequential row-store format, the baseline needs an additional stage to form 8K\x{}8K matrices before the compute kernel starts. In contrast, the alternate configuration with sub-block format already has 8K\x{}8K submatrices stored in main memory and does not require the CPU to prepare data for compute kernels. In figure~\ref{fig:cpu_overhead}(a), the sequential baseline configuration requires 2.11\x{} more time to avoid CPU overhead than the sub-block configuration does.

\noindent\textbf{[P2]: Underutilization of interconnect bandwidth.} 
%\cfigure[Figures/RDMA.pdf,{The effective bandwidth for different fetched data sizes through NVMe over fabric/PCIe interconnects},fig:rdma] 
As a result of the mismatching data layouts between storage and compute kernels, I/O requests to fetch data chunks are typically smaller than the sizes that can amortize the overhead of each I/O transaction, leading to underutilized interconnection bandwidth on the I/O side. In modern NVMe~\cite{NVMe11} interface, interconnect bandwidth saturates if each request is larger than 2~MB. However, when fetching a row containing 8K elements for an 8K\x{}8K submatrix (Figure~\ref{fig:conventionalStore}), each I/O request is for 32~KB of data, and the interconnect only achieves 66\% of the peak bandwidth. 

To maximize I/O bandwidth, an application may be designed to fetch consecutive chunks of storage data into a large memory buffer and gradually copy the buffered data into designated memory locations. However, the latter approach creates three performance issues: (1) it generates traffic from copying small data blocks on the CPU-memory bus, (2) it wastes precious main-memory capacity for memory buffers, and (3) it fetches data elements that the application might not use immediately and might need to fetch again due to limited buffer memory capacity and so wastes I/O bandwidth.

\ignore{
Figure~\ref{fig:rdma} shows the I/O bandwidth associated with fetching data sizes from NVMe (NVM Express) over fabric/PCIe (Peripheral Component Interconnect Express); interconnect bandwidth saturates if the request is larger than 2~MB. When fetchingc submatrices (Figure~\ref{fig:conventionalStore}), each I/O request is for 32~KB of data, and the interconnect only achieves 66\% of the peak bandwidth. In fact, an NVMe command can carry up to 32~MB of content to maximize the I/O bandwidth, but the application must still fetch and copy partial rows from one memory location to another for compute kernels, again underutilizing main-memory space and bandwidth.}

\noindent\textbf{[P3]: Underutilization of device bandwidth.} 
%\cfigure[Figures/SSDOverhead.pdf,{The relative execution time of matrix multiplications using row-store format (sequential) and sub-block format, with data in a 32-channel SSD},fig:ssd_overhead]
One-dimensional LBA space requires that an application materialize the original multi-dimensional data structure when presenting the data in storage. If the data dimensionality or the access pattern does not fit the storage device’s internal structure, the application consuming the materialized data is likely to underutilize the device’s internal bandwidth. As 
%illustrated 
in Figure~\ref{fig:conventionalStore}, when fetching 8K\x{}8K submatrices, a program can only utilize 50\% of the available parallel channels (device internal bandwidth) since the requesting data only reside in 4 of the 8 channels.

Figure~\ref{fig:cpu_overhead}(b) shows the impact of such underutilized bandwidth in a real application by extending the situation in Figure~\ref{fig:cpu_overhead}(a) for data placed in an SSD with 32 parallel channels. Besides the CPU overhead of transforming rows into submatrices, the baseline spends 1.92\x{} more time fetching data compared to an SSD configuration with optimal data layout for the workload by storing 8K\x{}8K submatrices consecutively due to the underutilized bandwidth.

\subsection{Challenges}
\label{sec:challenges}

Given the observations in Section~\ref{sec:conventional_model}, the data layout of an input dataset from memory/storage must fulfill the following requirements to fundamentally address the locality and dimensionality mismatch between storage data and compute kernels on hardware accelerators: (1) The layout must minimize the overhead of restructuring data in compute kernels and hardware accelerators. (2) The layout must allow the application to fully utilize the internal bandwidth of the storage device. (3) The layout must maximize the granularity of I/O commands and thus minimize the number of I/O requests.

Under the linear address space that a conventional storage system exposes, designing an optimal data layout that satisfies the above three requirements is challenging, for the reasons given below.

\cfigure[Figures/granularity.pdf,{The effective data processing rates or I/O bandwidth of system components with various matrix sizes},fig:granularity]
\noindent\textbf{[C1]: Unavailability of internal memory-device architecture to applications.} 
A storage device abstracts memory locations into LBAs without informing applications about the device structure. Existing NVMe commands allow an application to query the parameters of an underlying device and to optimize the LBA layout for an individual device; however, garbage collection and wear-level functions in the SSD management layer (including the flash-translation layer [FTL] and PCM translation layers~\cite{10.1145/1555754.1555759, 6296503,9138961}) can lead to data-location shuffling and suboptimal performance.

In addition, the application is unable to optimize the LBA layout for all storage devices because internal designs and hardware structures differ among devices. Consider Figure~\ref{fig:granularity}, which shows the data-processing rate or I/O bandwidth of each hardware component. %For storage devices, the data-processing rate is limited by the effective I/O bandwidth accessible to the application. Figure~\ref{fig:granularity} shows the data-processing rates 
For two flash-based SSDs, one with 32 channels and the other with only 8 channels, the 32-channel SSD can utilize the maximum bandwidth with the 512\x{}512 matrices that the application fetches (4~GB data sequentially from the SSD’s LBA space), but the 8-channel SSD only achieves its own maximum bandwidth (again, with 4~GB data fetched sequentially). Figure~\ref{fig:granularity} thus underscores the extreme difference in optimal data sizes due to different internal device architectures.

\noindent\textbf{[C2]: Unpredictability of optimal dimensionality in compute kernels. }
Because any applications can share a dataset, and a compute kernel can execute on a variety of computing resources, there exists no optimal layout that can maximize the efficiency of all applications or accelerators. For example, a row-oriented or column-oriented pair-wise matrix can maximize GPU computation, but cannot be efficient for matrix-multiplication kernels.

Figure~\ref{fig:granularity} also compares the data-processing rates and input-data sizes for processors/accelerators using different computation models---the vector processing model (used with general matrix multiply, GEMM, from Nvidia’s cuBLAS~\cite{cuBLAS} library) on conventional GPU cores (CUDA cores), and the 2-D matrix-processing model used with Nvidia’s Tensor Cores. To measure pure compute-kernel performance, we made all matrices available on the GPU device memory before the GEMM functions were invoked. Setting aside the significant performance lead in Tensor Cores, the optimal submatrix size that maximizes performance on the CUDA cores was found to be 2048\x{}2048, whereas the optimal submatrix size for the Tensor Cores was 512\x{}512.

\noindent\textbf{[C3]: Demand mismatch between storage devices and compute kernels. } 
Even though a user can narrow down the use of a dataset to a specific type of compute kernel, hardware accelerator, and dedicated storage device, there is no guarantee that the optimal input data for the hardware accelerator will match the layout that can fully utilize the internal bandwidth of the storage device. For the situation covered in Figure~\ref{fig:granularity}, our matrix-multiplication kernel worked best on 512\x{}512 submatrices, but the bandwidth for the consumer SSD is maximized if each I/O request fetches 16K\x{}16K submatrices. 
% (i.e., 4~GB of data).

%\CMF{
\subsection{Alternatives}
\label{sec:alternatives}
Prior work has addressed mismatching dimensionalities in modern computers through (1) more efficient data storage formats, (2) libraries supporting high-dimensional addressing, and (3) offloading of I/O operations to intelligent storage devices. Unfortunately, none of the three approaches tackles the challenges mentioned in Section~\ref{sec:challenges}. 

\noindent\textbf{File formats}
Much work has focused on dense data storage. Apache's Parquet~\cite{parquet} and ORC~\cite{ORC} 
offer efficient columnar storage formats, and Arvo~\cite{arvo} offers row stores for Hadoop. To 
reduce the CPU processing overhead of deserializing objects, Google's protocol buffers~\cite{ProtocolBuffer} 
and JSON's binary representation (BSON)~\cite{7765670} propose binary-encoded internal data 
representations. Albis~\cite{Trivedi2018AlbisHF} fuses features of columnar/row-major stores 
with binary-encoded formats to exploit both spatial locality and low-overhead deserialization. 
Domain-specific file formats are also available to address the demand of popular compute kernels 
in application subsets: aggregate genomic data (AGD)~\cite{203159} for biological applications, 
G-Store~\cite{kumar2016g} for graph applications, and JSOI~\cite{8904481} and ONNX~\cite{ONNX} for 
machine learning models. Frameworks that automatically generate data layout for GPU kernels~\cite{7877132,10.1145/2892208.2892210} also exist. None of these formats can address challenges posed by \textbf{[C1]} and \textbf{[C3]}, leading to problems \textbf{[P2]} and \textbf{[P3]}. 
% by hidden-device architectures underlying linear address-space abstraction, leading to demand mismatches between devices and unpredictable compute kernels \CMFcom{As intended?}.

\noindent\textbf{High-dimensional software I/O libraries}
To reduce the overhead in applications that create high-dimensional data objects, cloud storage systems such as N5~\cite{N5} and Zarr~\cite{Zarr} use high-dimensional addressing modes and chunk raw data to better utilize I/O bandwidth. Zarr~\cite{Zarr} also uses data compression to maximize the effective I/O bandwidth. These software libraries still only access abstracted linear memory/storage address spaces, which leads to problems \textbf{[P2]} and \textbf{[P3]}.
%under-utilization of device- or system-interconnect bandwidth.

\noindent\textbf{In-storage processing (ISP)}
To present data objects in a way that compute kernels require and improves the bandwidth/memory demand and CPU overhead, near-data processing (NDP) or ISP models can use a device’s internal bandwidth by working on the controller within the device. Existing ISP frameworks can transform rawdata into application objects for general-purpose compute kernels~\cite{KaleidoSSD}, mixed-precision/approximate computing workloads~\cite{ApproxSSD} or specialized applications like large graphs~\cite{matam2019graphssd}. However, the above approaches are all lacking in that ISP cannot efficiently produce application objects by fully utilizing interconnect bandwidth  (\textbf{[C3]}) unless the in-device data layout fits the access patterns of ISP code.
\ignore{
this approach improves the bandwidth/memory demand and CPU overhead because NDP models can deliver data that are ready for the compute kernels to use. Morpheus~\cite{KaleidoSSD} provides a framework for creating code that runs in an SSD to deserialize raw data into the required objects. GraphSSD~\cite{matam2019graphssd} offers a full system framework for storing, accessing, and operating graph analytics on SSDs. Varifocal Storage~\cite{ApproxSSD} allows applications to adjust the output from an SSD to data resolutions that optimize compute-kernel performance. However, the above approaches are all lacking in that ISP cannot efficiently produce application objects by fully utilizing interconnect bandwidth  (\textbf{[C3]}) unless the in-device data layout fits the access patterns of ISP code.}


\ignore{
%CMF: PREVIOUS VERSION
\label{sec:background}
One source of inefficiency of processing high-dimensional datasets in modern
computers is the mismatching dimensionalities of hardware accelerators,
memory devices and abstractions. This section explains why mismatching dimensionalities
affect application performance, the challenges of tackling the issue and how existing work falls short in
addressing the problems. 

% show the reasons of disadvantages.
\subsection{Modern accelerator-based architectures}
\label{sec:conventional_model}

Figure~\ref{fig:conventionalStore} illustrates the key hardware components
in modern heterogeneous computers for processing high-dimensional datasets.
In addition to the CPU and the main memory where the system controls the
application workflow and synchronizes data, a modern heterogeneous computer
typically uses hardware accelerators (e.g., GPUs in
Figure~\ref{fig:conventionalStore}) to perform compute kernels on high-dimensional
datasets. Modern GPUs provides two types of microarchitectures, the
conventional GPU cores that operate on vectors and Tensor Cores that operate
on matrices, to more efficiently process high-dimensional datasets. 

To provide high-performance data storage, the computer may use a solid state
drive (SSD) that stores data in non-volatile memory technologies (e.g., flash memory
and phase change memory [PCM]). All non-volatile memory technologies, have their own basic access 
granularities (e.g., page in flash memory). This is even true for emerging devices like
PCM~\cite{WuUnwrittenContract3DXPoint}. To improve the bandwidth, modern
SSD controllers exploits channel-level and bank-level parallelism. Modern SSDs typically organize 
their memory arrays into channels where all parallel channels can accept unique requests 
simultaneously. Each channel also contains multiple banks that a free bank
can accept a request while other banks are busy. As commercialized non-volatile memory
technologies have limited program-erase cycles, SSD controllers must also
carefully manage the mapping between logical address that the software views
and the physical memory locations. 

As modern storage systems still expose linear address spaces (e.g., logical
block addresses [LBAs]) to the rest of the world, producers of
high-dimensional datasets must reduce data dimensionality to 1-D
representations like row-oriented or column-oriented storage formats. If a hardware-accelerated
compute kernel needs to compute on datasets, the application invoking the
compute kernel must first fetch the each piece of necessary data from the storage
system. Then, the application assembles each received piece into memory
objects with a layout that satisfies the demand of the target accelerator's architecture.
Finally, the application copies the created memory object from the host main
memory to the accelerator's device memory for compute kernels. 

Figure~\ref{fig:conventionalStore} also shows the process of performing
matrix multiplications (MM) using a modern GPU. The GPU kernel delivers maximum throughput
of computation if the MM kernel is performed on 8K\x{}8K sub-matrices. The origin dataset presents their
matrix inputs using a row-oriented storage format, as the format is
generally considered the most efficient for CPU-based compute kernels. The
size of the raw input matrices are 16K\x{}16K. The SSD has 8K pages and 8 parallel
channels. Therefore, each SSD page will store 2K elements encoded in the IEEE-754 32-bit floating
point format and each row of a matrix will occupy 8 pages that are logically consecutive
in LBAs. In conventional SSD design, these consecutive pages are
typically stripping across different channels to enable parallel
accessing for sequential accesses in LBAs, since most file systems and
applications still assume their underlying storage devices are more
efficient when performing sequential accesses. Therefore, the physical
locations of these 8 pages belonging to the same row will locate in distinct channels. 

To
maximize the efficiency on machines with limited high-speed memory capacity available 
to the hardware accelerator, the application must create a pipeline to logically partition 
input matrices into sub-matrices and perform multiplications on pairs of
sub-matrices. In each pipeline, the application must first create a sub-matrix
by retrieving necessary elements from all involved rows into the destination
location in the system main memory. After all elements of a submatrix
arrived, the application copies the created submatrix to the accelerator's
device memory and finally launches the comupte kernel depending on the
copied submatrice. This example also shows several deficiencies of resulting
from the mismatching demand between modern
hetergeneous computing units and linear addressing of the storage system. 

\cfigure[Figures/CPUOverhead.pdf,{The relative execution time of matrix
multiplications using row-store format (sequential) and sub-block format,
assuming data is already in the main memory},fig:cpu_overhead]
%\hungwei{Definitely need to revise the followings}
%\vspace*{-0.2in}
\textbf{The overhead of reshaping input data} 
To reshape stored data into 
the desired dimensionality in hardware accelerators, the application must
use CPU instructions to calculate the mapping between the raw data offset
and the target memory locations. Then the application must issue I/O requests 
through system software stack, again using CPU instructions, to fetch pieces 
of raw data and place (potentially also convert) 
received data pieces in their designated memory locations. In the example of 
Figure~\ref{fig:conventionalStore}, if the application needs to fetch an
8K\x{}8K submatrix, the row store format will require the program to issue
8,192 I/O requests to fetch 8,192 rows that contain the items for the
submatrix. 

Figure~\ref{fig:cpu_overhead} illustrates the CPU overhead. In
Figure~\ref{fig:cpu_overhead}, the raw data already presented in the system
main memory before the compute kernel launches. The system uses an AMD RyZen
3700X CPU and NVIDIA's RTX 2080 GPU. The baseline is pipelined matrix 
multiplications of multiplying two 32K\x{}32K matrices using sub-blocks of 8K\x8K
matrices. However, as the source dataset uses sequential, row-store format, the
baseline needs an additional stage to form 8K\x{}8K matrices before a
compute kernel starts. In constrast, the other configuration, sub-block,
already has 8K\x{}8K sub-matrices stored in the main memory and does not
require CPU to prepare data for compute kernels. The result
shows that the baseline spends 2.11\x{} more time than the configuration
avoiding CPU overhead. 
%\hank{Can we have some data showing the overhead?}

\textbf{Under-utilizing the interconnect bandwidth} 
\cfigure[Figures/RDMA.pdf,{The effective bandwidth of fetching data in
different sizes through NVMe over fabric/PCIe interconnects},fig:rdma]
As a result from the
mismatching data layouts on storage and compute kernels, the I/O requests
of fetching chunks are typically smaller than the sizes that can amortize
the overhead of each I/O transactions, leading to under-utilized
interconnection bandwidth on the I/O side. To maximize the I/O bandwidth,
another way to compose an application is to fetch consecutive storage data 
into a large memory buffer and gradually copy buffered data into their designated memory
locations. However, the later approach also create three performance issues.
(1) It generates traffic in copying small data blocks on the CPU-memory bus.
(2) It wastes precious main memory capacities for memory buffers. 
(3) It fetches data elements that the application potentially will not use
within a short period of time and wastes the I/O bandwidth.

Figure~\ref{fig:rdma} shows the I/O bandwidth of fetching various sizes of
data from NVMe over fabric/PCIe. The interconnect bandwidth saturates if the
request is larger than 2~MB. 
In the example of Figure~\ref{fig:conventionalStore} in fetching 8K\x{}8K
submatrices, each I/O request is simply requesting 32~KB of data and the
interconnect only achieves 66\% of the peak bandwidth. In fact, an NVMe
command can carry up to 32~MB of content to maximize the I/O bandwidth. 
However, the application still has to fetch and copy partial
rows from one memory location to another for compute kernels and again,
under-utilizing the main memory space and bandwidth. 

%\hank{Any data showing the RDMA I/O bandwidth is saturated with larger I/O requests?}

\textbf{Under-utilizing the device bandwidth} 
\cfigure[Figures/SSDOverhead.pdf,{The relative execution time of matrix
multiplications using row-store format (sequential) and sub-block format,
assuming data is in a 32-channel SSD},fig:ssd_overhead]
Due to the one-dimensional LBA space, an application must materialize the
original multi-dimensional data structure into a selected dimension when
presenting the data in storage. If the size of a dimension or the access
pattern on the selected dimensional does not fit the storage device's internal
structure, the application consuming the materialized data are very likely
to under-utilized the device's internal bandwidth.
%As the SSD hides their internal multi-dimensional
%structure and , 
In the example of Figure~\ref{fig:conventionalStore} in fetching 8K\x{}8K
submatrices, the program can only utilize 50\% of the parallel channels
(i.e., 50\% of the device internal bandwidth) since the requesting data only 
reside in 4 of the 8 channels. 

Figure~\ref{fig:ssd_overhead} shows the impact of such under-utilized bandwidth
in an real application. Figure~\ref{fig:ssd_overhead} extends the
experiments in Figure~\ref{fig:cpu_overhead} by placing data in an SSD with
32 parallel channels. The baseline spends 2\x{} more time than storing
sub-blocks in the SSD and fetching sequential data in the baseline takes 1.92\x{} more
time than the sub-block format due to the under-utilized format. 

% -- Reshaping overhead: CPU instructions to calulate addresses and issue I/O
% requests, increased amount of I/O accesses, prevents P2P connections, 
% -- Inefficient use of device bandwidth: row/column access order, internal
% parallelism due to conflict of channels and banks. 
% Challenges. 
% -- Mismatching shapes: the best shape of each accelerator, compute kernels
% and storage are different.
% -- Cannot predict the compute kernel
%\subsubsection{The overhead of reshaping data}
%\label{sec:reshaping}

\subsection{Challenges}
\label{sec:challenges}
Through our observations in Section~\ref{sec:conventional_model}, the data
layout of an input dataset must fulfill the following properties to fundamentally 
address the deficiency of the mismatching locality and dimensionality between storage 
data and compute kernels on hardware accelerators. \\
(1) The
layout must minimize the overhead of reshaping data in compute kernels and
hardware accelerators. \\
(2) The layout must allow the application to fully
utilize the internal bandwidth of the storage device. \\
(3) The layout must
maximize the granularity of I/O commands and thus minimize the number of I/O
requests. \\
However, under the linear address space that conventional storage system
exposes, designing a perfect data layout that holds the above three properties
is challenging.

\cfigure[Figures/granularity.pdf,{The effective bandwidth of fetching data in
different sizes through NVMe over fabric/PCIe interconnects},fig:granularity]
%\vspace*{-0.2in}
\textbf{The internal architecture of memory device is hidden from applications} 
As the
storage device abstracts the memory locations into LBAs, the device structure
and characteristics are hidden from applications. 
Even though existing NVMe
commands allow the application to query parameters of the underlying device
and optimize the layout on LBAs, the address remapping, garbage collection,
wear-level functions in an SSD management layer, including flash 
translation layer (FTL) and PCM
translation layers~\cite{10.1145/1555754.1555759, 6296503,9138961}, will
shuffle the data locations and still lead to sub-optimal performance. 

In
addition, the application can never optimize the layout for all storage devices
as the internal design and the hardware structure differ from device to
device.
Figure~\ref{fig:granularity} shows the data processing rate of each hardware
component. For storage devices, the data processing rate means the effective I/O
bandwidth observed by the application. In Figure~\ref{fig:granularity}, we
present two flash-based SSDs, one with 32 channels and the other with only
8 channels. The 32-channel SSD achieves the maximum bandwidth with
512\x{}512 matrices that the application fetches 4~MB data sequentially from
the SSD's LBA space, but the 8-channel SSD needs fetches 4~GB data sequentially
to achieve its maximum bandwidth. This result shows the huge difference in
optimal data sizes due to the difference in their internal architectures. 

%\vspace*{-0.2in}
\textbf{The unpredictability of optimal dimensionality in compute kernels}
As many applications can share a dataset, or a compute kernel can
potentially execute on various types of computing resources, there exists no optimal
layout that can maximize the efficiency of all applications or accelerators.
For example, either row-oriented or colume-oriented for pair-wise matrix can
maximize the computation on GPUs, but cannot be efficient for matrix
multiplication kernels. 

To prove this argument, Figure~\ref{fig:granularity} also compares the data processing rates, the
amount of input data that the highly optimized General matrix multiply
(GEMM) from NVIDIA's cuBLAS~\cite{cuBLAS} library on conventional GPU cores
(CUDA Cores) using the vector processing model and Tensor Cores using the
2-D matrix processing model. To measure the pure compute kernel performance,
we make all matrices available on the GPU device memory before GEMM
functions are invoked. Aside from the significant performance lead in
Tensor Cores, the optimal sub-matrix sizes that maximize the performance on
CUDA Cores and Tensor Cores are also different, 2048\x{}2048 for CUDA Cores
but 512\x{}512 for Tensor Cores. 


%\vspace*{-0.2in}
\textbf{The mismatching demand between storage devices and compute
kernels} 
Even though the user can narrow down the use of a dataset to a
specific type of compute kernel and a hardware accelerator as well as a
dedicated type of storage device, there is no guarantee of that the optimal
shape of input data for th hardware accelerator will match the layout that
can fully utilize the internal bandwidth of the storage device. 
For Figure~\ref{fig:granularity}, our matrix multiplication kernel works the best
on 512\x{}512 submatrices, but a consumer SSD maximizes its internal
bandwidth if each I/O request fetches 4~GB of data (i.e., 16K\x{}16K
submatrices). 

\subsection{Alternatives}
\label{sec:alternatives}
% HANK: need to use label.
Prior work has been addressing the mismatching dimensionalities in modern
computers through (1) more efficient data storage formats (2) library
supporting high-dimensional addressing and (3) offloading I/O operations to intelligent storage devices.
However, all three approaches failed to tackle the challenges Section~\ref{sec:challenges}
mentions. 

\textbf{File formats}
There has been a plenty of works focusing on dense data storage in different scenarios.
Apache's Parquet~\cite{parquet} and ORC~\cite{ORC} offer efficient columnar storage formats
as well as Arvo~\cite{arvo} offers row store for Hadoop. To reduce the
CPU processing overhead in deserializing objects, Google
s protocol buffers~\cite{ProtocolBuffer} and JSON's binary~\cite{7765670}
propose binary-encoded internal data representations. 
Albis~\cite{Trivedi2018AlbisHF} fuses the features from columnar/row-major
stores with binary-encoded formats to exploit both spatial locality and low-overhead
deserialization. 
There also exists domain-specific file formats address the demand of
popular compute kernels in a particular set of applications, including Aggregate Genomic 
Data (AGD)~\cite{203159} for biological applications, G-Store~\cite{kumar2016g} for graph
applications, JSOI~\cite{8904481} and ONNX~\cite{ONNX} for machine learning models.
There are also frameworks that automatically generates data layout for GPU
kernels~\cite{7877132,10.1145/2892208.2892210}. 
However, none of these formats can address challenges from the hidden device
architecture behind linear address space abstraction, mismatching demand of devices and 
unpredictability of compute kernels. 


\textbf{High-dimemsional software I/O library}
% High-dimensional storage
The reduce the overhead in applictions in creating high-dimemsional data
objects, cloud storage systems including N5~\cite{N5}, Zarr~\cite{Zarr}, offer 
high-dimensional addressing mode and chunk rawdata to better utilize I/O bandwidth. Zarr~\cite{Zarr}
additionally implements data compression for maximize effective I/O
bandwidth. However, these software library solutions still see only abstracted linear memory/storage
address spaces and lead to under-utilization of device or system
interconnect bandwidth. 
%N5~\cite{N5} is a storage interface that offers high-dimensional APIs 
%specifing the primitive operations needed to store large chunked n-dimensional tensors, 
%and arbitrary meta-data in a hierarchy of groups. 
%Zarr~\cite{Zarr} not only offers a high-dimemsional indexing mode, but also provide 
%an implementation of compressed, chunked, N-dimensional arrays for high-dimensional data storage.
%However, N5 and Zarr require programmers to configure parameters of storage formats and devices, 
%and this may still lead to a sub-optimal performance because of misconfigurations.
%Compared to N5 and Zarr, \NDS{} is transparent to programmers to guarantee the optimized, agnostic I/O performance to underlying systems. 

% Sparse formats
%\paragraph{Sparse data representations}
%Compared to those works, \NDS{} not only focuses on offering an high-dimensional addressing mode to support data representation, 
%but also optimizing the efficiency of device's hardware resources.

\textbf{Near-Data Processing}
% Other Near-Data Processing Approaches 
To present data objects in a way
that compute kernels desire, near-data processing (NDP) model can more
efficiently use devices' internal bandwidth as NDP works on the controller
within the device but also improves the bandwidth/memory demand as well as
CPU overhead since NDP model can deliver data that are ready for the compute
kernels to use. Morpheus~\cite{KaleidoSSD} provides a framework that allows
programmer to create code running in an SSD to deserialize raw data into the
desired objects.  GraphSSD~\cite{matam2019graphssd} offers a full system
framework for storing, accessing and operating graph analytics on SSDs. 
VarifocalStorage~\cite{ApproxSSD} allows applications
to adjust the output from the SSD to data resolutions that otimizes the compute kernel
performance. However, if the in-device data layout does not fit the access
pattern of in-storage processing code, NDP still cannot efficiently produce
application objects and fully utilize the interconnect bandwidth. 
%Near-Data Processing (NDP) is a concept of processes data in memory or in storage to 
%reduce the transfer overhead and the stress on the host CPU. 
}
\ignore{

\subsection{missing high-dimensional indexing}
Because the traditional hardward components are 0-D or 1-D,
the common addressing mode only requires programmers offer an offset and a length in one direction for I/O operations.
However, with many high-dimensional applications come up, 
there are lots of high-dimensional hardware accelerators, 
such as NVIDIA's TensorCore or Google's Tensor Process Unit, available in the market.

Usually, those hardware accelerators require programmers to 
manually prepare a piece of 2-D submatrix from a big matrix,
transfer to the memory in hardwares, invoke compute kernels and get results.
During the preparation, programmers have to use traditional 1-D addressing mode to
request 2-D or higher dimensional data. 
For example, programmers have to calculate the offset and the length of the first row of the submatrix.
Next, ones have to pay attention on the offset of the second row of the submatrix from the rawdata to get it correctly, and so on so forth.
These extra efforts would make applications more error-prone or 
force programmers to spend more time on checking the correctness of address calculation.

There are some functions, such as cudaMemcpy2D, trying to handle fetching 2-D data.
However, those functions still require programmers to offer 1-D address firstly,
and they will handle the rest of operations.

Some libraries offer multidimensional indexing that allows users to read/write high-dimensional data.
However, since underlying implementations is still in 1-D address mode, 
programmers have to check the shape of the source and 
the shape of the destination are the same before doing any I/O on them. 
Also, those multidimensional indexing assume programmers would work on single element-wise object in the data,
so the default granularity of this indexing is 1.
However, in our observations from applications, 
the granularity of reading/copying/calculating submatrices from the rawdata is usually larger than 1,
so the memory bandwidth and the ALU units can be fully utilize.
If programmers want to change the granularity of submatrice, 
they have to pay attention on rewriting the starting and ending index to get the correct shape of data.
This would cause an extra effort and make application error-prone.

\subsection{Overhead of reshaping data}
% Hardware is not the most critical bottleneck in many applications.
% However, those accelerators introduce reshaping because of multi-dimension data requirement

With Google's TPU or Nvidia's TCU, we are able to operate Matrix Multiply-Accumulate (MMA) faster
than conventional GPU approach. However, those hardwares requires data being in two-dimension, which
leads an overhead of reshaping serialized data from 1D to 2D.

However, those hardwares requires two-dimensional sub-matrices, which usually are a few rows and a 
few columns of the original data. Although modern NVM-based SSDs is able to handle multiple, fixed-sized
requests in parallel through the internal channels, if the file is stored in conventional row/column-store, 
it would increase the probabilities of competing channels and thus under-utilize internal parallism.

% put the figure 5 in CNS proposal here.
Figure shows a simplified example of data layouts and SSD channels to compare tensor-store format and conventional row-store format.
Figure (a) represents the logical view of a 16x16 matrix which can be partitioned into 16 submatrices, and each submatrix contains 4 rows and 4 columns.

If the simplified SSD has 4 parallel channels and each page can only fill in a half row of the matrix, by using conventional row-store format, it would
strip each row across two channels as in Figure (b). If a tensor operation requests submatrix \#1 from the SSD, with the conventional row-store, 
the SSD has to fetch the first half of the first 4 rows where only channel \#1 and channel \#3 contain the requested data. As a result, the SSD needs to
issue 4 requests, but only two of them can be executed in parallel.

With the tensor-store layout as Figure (c), each SSD page stores half of a submatrix. In this case, the SSD simply needs 2 requests on 2 parallel channels
to fetch submatrix \#1. Compared to the conventional row-store format, the speedup on I/O is 2x. Furthermore, this submatrix can be considered as a "building block."
For example, if a tensor operation needs a 8x8 submatrix at the upper-left corner, \NDS{} is able to reassemble submatrices \#1, \#2, \#5 and \#6 into a larger matrix,
and the resulting submatrix should be co-located instead of following the original logical locations.

In the real-world scenarios, the speedup achieved by the tensor-store format is more significant than the example in Figure.
Unlike the conventional storage format that stores values from the same row or the same column within the same 8KB page, 
tensor-store format fills the page with a logically adjacent 32x32 double-precision submatrix. In a case that an application requests
a 256x256 submatrix from an SSD with 8 KB pages and 8 internal channels, the conventional storage format can only utilize the half of the SSD's channels.
Nevertheless, the tensor-store format is able to use all channels in the SSD and only has to issue 8 serialized commands in each channel.
This results in 8x I/O speedup without any changes in hardwares.

% For example, (shows the description and figures in proposal.)
\subsection{Inflexibility of preprocessed data}
One way to avoid reshaping overhead during the application runtime is proprecessing rawdata beforehand.
There are many preprocessing approaches, such as flattening or batching. 
Based on the current hardware/software stacks, programmers
would profile the efficiency to decide the reshaped size of data or the batch size.

Take the field of image classification as an example, before running the computation,
each image is firstly flatten from a 2-D matrix to an 1-D array to avoid the overhead of reshaping. 
Next, those preprocessed 1-D arrays are concatenated together as one file object, 
so applications can read batched data to avoid lookup overhead.

However, current high dimensional hardware accelerators 
have diffenent designs and architectures to achieve a similar operation.
According to the documentation, the recommended shape for TPU is 256x256, 
but the recommended shape for TCU is 16x16.

As a result, although we could reshape data to a desired format to avoid mentioned overheads, 
once the system are changed, programmers might still have to reshape the preprocessed data 
to an another shape during or before the application runtime to reach the same or 
a better performance.
 
\subsection{Different Devices need different granularity}
Conventional I/O APIs allow programmers to adjust IO size to maximize the I/O throughput.
However, a modern computer usually owns a heterogeneous accelerator (e.g. GPU or FPGA) and a modern storage device (e.g. NVMe SSD) connected by PCIe or RDMA.

Although these modern hardwares significantly reduce the end-to-end latency of applications, they complicates the system configurations. 
Without knowledge and exhaustive searches, improper parameters might lead to suboptimal performance of applications. 

For instance of running the GEMM application on our baselined system, a GPU kernel has the best goodput when the shape of input
matrix is 2048x2048. However, if a user naively requests a 2048x2048 submatrix from the storage device, the shape of the requested
matrix is not favorable size of the storage device and thus leads a significant latency and a sub-optimal performance. 

To achieve the best I/O performance, firstly one should exhaustively find out the most suitable configuration in the storage device.
Next, the parameters of interconnect between the host machine and the storage device must be resolved as well.

From the figure, fetching a 256x256 matrix from the storage device gives a lower response time and thus leads 
the best end-to-end latency of an application. Moreover, the highest bandwidth threshold is achieved when 
sending 512 elements message through interconnect between the host machine and the storage device. 

However, one should remind that this parameters are dependent on the storage infrastructure. As a result, we proposed a full-stack
storage system that hides the complexity behind programmers. No matter what the granularity resulting in the
best computing gootput is chosen, because of highly-optimized storage backend, it is still able to offer applications the best I/O bandwidth.


% \ignore{
% Traditionally, we store data in the one-dimensional format, we have to
% reshape the data to a desired dimensional format for applications.

% When another
% application needs to retrieve data, the application must
% also reshape the serialized data to the desired dimension.

% GPUs need matrix shape
% How to show under-utilize bandwidth? Check proposal?
% GEMM(?)

% First, as the
% application must always reshape data for compute kernels
% on accelerators, the application is very likely to under-utilize
% the hardware accelerators as the goodput of generating reshaped
% data from one-dimensional data layout is generally
% slower than the throughput of accelerators.

% \subsection{Overhead of row-/column-accesses}
% Beside the overhead of reshaping data, reassembling one-dimensional data to two-dimensional matrix
% needs multiple row accesses, which can lead to under-utilized bandwidth.

% (check proposal here to see how to describe the problem.)
% }
% (also we can refer other works related to format)

To address mentioned problems, we proposed \NDS{}, which is an end-to-end storage framework that stores/fetches high-dimensional data
for high-dimensional applications.

In this work, we borrowed the concept of the chunked storage, which make a better utilization of internal channels of SSDs. 
Also, \NDS{} offers a set of APIs that allow programmers to rebuild the desired shape from building blocks.
\NDS{} hides complex parameters from programmers and is implemented a software pipeline to achieve the best I/O performance.
Finally, to alleviate the CPU loading, we implemented a version that puts the storage backend onto the storage device.

% introduce each section.


\ignore{
Needed granularity by applications are different. (cited paper?)

Third, even though the data is already
presented in some optimal, high-dimensional data layout, the
desired shapes are still different from applications to applications.
}

\ignore{
A typical computer system contains one or more
processors with DRAM-based main memory and stores the bulk data
as files in storage devices.  Because of SSDs' high-speed, low-power, and
shock-resistance features, the system may use flash-based SSDs
as the file storage. The system may also include GPU
accelerators that contain thousands of Arithmetic Logic Units (ALUs) to provide vectorized
parallelism. These SSDs and GPUs connect with the host computer system
through the Peripheral Component Interconnect Express (PCIe)~\cite{PCIe}
interconnect. These SSDs communicate using standards including
Serial Advanced Technology Attachment (Serial ATA or SATA)~\cite{SATA} or NVM Express
%or Non-Volatile Memory Host Controller Interface Specification
(NVMe)~\cite{NVMe, NVMe11}. These
standards allow the host computer to issue requests to the storage device, including reads,
writes, erases, and some administrative operations.

To exchange, transmit, or store data, some applications use
data interchange formats that serialize memory objects into ASCII
or Unicode text encoding (e.g. XML,
CSV, JSON, TXT, YAML). Using these text-based encodings for data
interchange brings several benefits. For one, it allows machines with
different architectures (e.g. little endian vs. big endian) to exchange
data with each other. These file formats allow applications to create their
own data objects that better fit the computation kernels without requiring
knowledge of the memory layout of other applications.  These text-based
formats also allow users to easily manage (e.g. compare and search)
the files without using specific tools.
However, using data from these data interchange formats also
results in the overhead of deserializing
%\Bella{(I deleted 'unmarshalling' because the term isn't used anywhere else in the paper)}
application objects, since it requires the computer to convert data strings into
machine binary representations before generating in-memory data structures from these
binary representations.


%\cfigure[Figures/conventional_model.pdf, {Object deserialization in
%conventional models},fig:conventional_model]
\dcfigureSingleCol[Figures/conventional_dataflow_model.pdf,Figures/conventional_model.pdf, {Object deserialization in
conventional models},fig:conventional_model]

Figure~\ref{fig:conventional_model} illustrates the conventional
%programming and execution
 model (Figure~\ref{fig:conventional_model}(a)) and
the corresponding data movements (Figure~\ref{fig:conventional_model}(b))
for deserializing application objects.
The application begins object deserialization by requesting the input data
from the storage device as in phase A of
Figure~\ref{fig:conventional_model}(a). After the storage device
finishes reading the content of the input file, the storage device sends the raw
data to the main memory through the I/O interconnect, resulting in the data
transfer from the SSD to the main memory buffer X as in arrow (1) of
Figure~\ref{fig:conventional_model}(b).
In application phase B of Figure~\ref{fig:conventional_model}(a), the application
loads the input data from the main memory (data transfer (2) in
Figure~\ref{fig:conventional_model}(b)), converts the strings into binary representations,
and stores the resulting object back to another location in the main memory (data transfer (3)
from the CPU to memory location Y in Figure~\ref{fig:conventional_model}(b)). The program may
repeat phases A and B several times before retrieving all necessary data.
Finally, the CPU or the graphics accelerator on an APU (Accelerated Processing
Unit (APU)~\cite{AMDAPU} can start executing the computation kernel which consumes the application
objects in the main memory as in phase C (data transfer (4) loading data from memory location Y
in Figure~\ref{fig:conventional_model}(b)). If the application executes the
computation kernel on a discrete GPU (use phase C' instead of C), the GPU needs
to load all objects from the main memory before the GPU kernel can begin (hidden lines of
Figure~\ref{fig:conventional_model}).

\cfigure[Figures/significance.pdf, {The overhead of object deserialization
in selected applications},fig:io_breakdown]
%\input{tableEffectiveBandwidth}

%Deserializing objects using the conventional model brings several drawbacks
%in application performance.
Because of the growing size of input data and intensive optimizations in
computation kernels, deserializing application objects has become a significant
performance overhead. Figure~\ref{fig:io_breakdown} breaks down the
execution time of a set of applications that use text-based encoding as their
input data. (Section~\ref{sec:methodology} provides more details about these
applications and the testbed.) With a high-speed NVMe SSD, these applications
still spend 64\% of their execution time deserializing objects. To figure
out the potential for improving the conventional object deserialization
model, we perform detailed experiments in these benchmark applications and
obtain the following observations:

\myitem{{Object deserialization is CPU-bound.}}
\cfigure[Figures/effective_bandwidth.pdf, {The effective bandwidth of object deserialization
in selected applications using different storage devices under different CPU
frequencies},fig:effective_bandwidth]
To examine the correlation between object deserialization and the speed of storage
devices, we execute the same set of applications and load the input data from
a RAM drive, an NVMe SSD, or a hard drive. The NVMe SSD can sustain more than
2~GB/sec bandwidth and the hard drive provides 158~MB/sec bandwidth. We
create a 16GB RAM drive using the host system DRAM attached to a DDR3 memory
bus that theoretically can offer up to 12.8~GB/sec bandwidth.

Figure~\ref{fig:effective_bandwidth} reports the effective bandwidth of
object deserialization for each I/O thread in these applications. In this paper, we
define the effective bandwidth as the memory size of application objects that the
system can produce within a second.
Compared to the traditional magnetic hard drive,
the NVMe SSD delivers 5\% higher effective bandwidth when using a 2.5~GHz Xeon
processor. However, the performance of the RAM drive is essentially no better
than the NVMe SSD. If we under-clock the CPU to 1.2~GHz, we observed
significant performance degradation. However, the performance differences
among different storage devices remain marginal.

This result indicates that CPU code is the bottleneck
when systems with high-speed storage devices deserialize objects from files.
In other words, if we use the conventional model for object deserialization in these
applications, the application does not take advantage
of higher-speed storage devices, even those as fast as a RAM drive.

\myitem{{Executing object deserialization on the CPU
is expensive.}}
To figure out the source of the inefficiency, we profile the code used to parse
a file of ASCII-encoded strings into an array of integers. The profiling result
shows that the CPU spent only 15\% of its time executing the code of
converting strings to integers. The CPU spent the most of  the rest of its time
handling file system operations including locking files and providing POSIX
guarantees.

The conventional approach to object deserialization also results in increased context
switch overhead. In the conventional approach, applications must access
the storage device and the memory many times when deserializing objects.
As a result, the system must frequently perform context switches between kernel
spaces and different processes since fetching data from the storage device or
accessing memory data can lead to system calls or latency operations.
For example, if a memory access in phase B of
Figure~\ref{fig:conventional_model}(a) misses in the last-level cache or if the
memory buffer in phase B needs to fetch file content, the system may switch
to the kernel space to handle the request from the application.

\myitem{{Object deserialization performs poorly on CPUs.}}
To further investigate the potential of optimizing the object
deserialization code, we implemented a function that maintains the same
interface as the original primitive but bypasses these overheads. Eliminating these
overheads speeds up  file parsing by 1.74~\x{}. However, the instruction-per-cycle (IPC)
of the remaining code, which examines the byte arrays
storing the input strings and accumulates the resulting values, is only 1.2. This
demonstrates that decoding ASCII strings does not make wise  use of the rich
instruction-level parallelism inside a CPU core.
%\Bella{ok?}

\myitem{{Deserializing objects using CPUs wastes bandwidth and memory.}}
The conventional object deserialization model also creates
unnecessary traffic on the CPU-memory bus and intensifies main
memory pressure in a multiprogrammed environment.

Deserializing objects from data inputs requires memory access to the input
data buffer and the resulting object locations as shown in phases A and B of
Figure~\ref{fig:conventional_model}(a) and steps (2)--(3) in
Figure~\ref{fig:conventional_model}(b). When the computation kernel begins
(phase C of Figure~\ref{fig:conventional_model}(a)), the CPU or a
heterogeneous computing unit (e.g. the GPU unit of an APU)
needs to access deserialized objects. This results in memory accesses to
these objects again. Since the computation kernel
does not work directly on the input data strings, storing the raw data in the memory
creates additional overhead in a multiprogrammed environment.
For APU-based heterogeneous computing platforms in which heterogeneous
types of processors share the same processor-memory bus, these memory
accesses can lead to contentions and degrade
performance of bandwidth hungry GPU applications~\cite{JasonHSC,RodiniaBenchmark}.

Since text-based encoding usually requires more bytes than binary
representation, the conventional model may consume larger bandwidth to
transport the same amount of information compared to binary-encoded
objects. For example, the number ``12345678'' requires at least 8
bytes in ASCII code, but only needs 4 bytes using 32-bit binary
representation.

\myitem{{Conventional object deserialization prevents applications from
using emerging optimizations in heterogeneous computing platforms.}}
Many systems support  P2P communication between two endpoints in the same PCIe
interconnect, bypassing the CPU and the main memory overhead~\cite{PCIe,DirectGMA, GPUDirect, GPU-Infiniband,
GPUP2Pcluster,GPUCommunication, 6012914, GPU-intranode, 6702638, 6587715, BittnerDirectGPUFPGA,
ZeroCopy, NVMMU, shihab2014gpudrive, gullfoss}. the conventional model restricts the usage of this emerging technique in
applications. Applications that still rely on the CPU-centric object deserialization
model to generate vectors for GPU kernels must go through every step
in Figure~\ref{fig:conventional_model}(b), but cannot directly send data from the
SSD to the GPU.
%\Bella{(This sentence looks more like a description than an explanation, so I took out the ``this is because'' phrasing.)}
This model also creates huge traffic
in the system interconnect and CPU-memory bus as it exchanges application
objects between heterogeneous computing resources.
\\
\\
In the rest of the paper, we will present and evaluate the \KaleidoStorage{} model that
addresses the above drawbacks of deserializing objects in the conventional
computation model.
}
}}


==> codeSimpleMM.tex <==
\begin{figure}
    \lstset{language=c}          % Set your language (you can change the language for each code-block optionally)
    \centering
    \begin{minipage}[b]{1\linewidth}
    \lstset{language=C,label=SliceExaple}
    \begin{lstlisting}[frame=single, mathescape,label=scopingExample]
void simple_16_16_16(float* D, half* A, half* B ) {
  simd2::matrix<simd2::matrixa,16,16,16,half> mat_A;
  simd2::matrix<simd2::matrixb,16,16,16,half> mat_B;
  simd2::matrix<simd2::accum,16,16,16,float> mat_C;
  simd2::fillmatrix(mat_C, 0.0f);
  simd2::loadmatrix(mat_A, A, 16);
  simd2::loadmatrix(mat_B, B, 16);
  simd2::mmo(mat_C, mat_A, mat_B, mat_C,minplus);
  simd2::storematrix(D,mat_C, 16);
}
\end{lstlisting}
\end{minipage}
\vspace{-0.12in}
\caption{Simple fixed shape min-plus MM with supppotr of 16$\times$16$\times$16 \SIMDD{} instrctions}
\label{code:simplemm} 
\vspace{-0.22in}
\end{figure}


==> others.tex <==
\subsection{Alternatives to Tensor Processing Units}
\label{sec:other_accelerators}

In addition to TPUs, the research community has presented hardware
accelerator architectures to improve tasks in AI/ML workloads. Similar to
the microarchitecture of TPUs, HyGCN~\cite{HyGCN}, Caffeine~\cite{Caffeine}, 
Gemmini~\cite{Gemmini}, Chain-NN~\cite{Chain-NN}, SCALE-Sim~\cite{SCALE-Sim}, Tensaurus~\cite{Tensaurus}, Eyeriss~\cite{Eyeriss}, Tangram~\cite{Tangram}, SNNAP~\cite{SNNAP}, Wei et al.~\cite{auto} and Kung et al.~\cite{PSCNN} all adopt systolic array based design. 

MAERI~\cite{MAERI}, FlexFlow~\cite{FlexFlow} ,TIE~\cite{TIE} and Song et al.~\cite{song2018towards} 
explore the parallelism of ML models' dataflow and re-design the PE layout in accelerator.
Shortcut Mining ~\cite{ShortcutMining} reuses shortcut data in NN models by buffering scheme to reduce off-chip data movement.
Simba~\cite{Simba} balances workload and reduces inter-chiplet communication of a MCMs system to acheive scalability.
VIP~\cite{VIP} couples with a 3D-stacked memory system to alleviate high memory demand.

% This paragraph should discuss NN accelerators not using systolic array,
% but still have matrices as inputs/output
%\jay{Besides systolic array, x and xx and xxx use whatever architecture to
%solve NN problems (If you have more than one architectures, mimic the
%formation and keep going)}.

%\jay{you can go through \url{https://www.dropbox.com/s/q3moiqcrhwf1pyc/1-s2.0-S2095809919306356-main.pdf?dl=0}
%for some ideas.}

Instead of implementing NN accelerators as a separate chip, recent advances
in near-data/in-memory processing allows the data-intensive NN computation
to occur without explicitly moving data through bandwidth limited system
interconnects. Neural Cache~\cite{NeuralCache}, TensorDIMM~\cite{TensorDIMM}, Manna~\cite{Manna}, Wang  et al. ~\cite{BPICA}, Liu et al.~\cite{PIM}, and Imani et al.~\cite{DLANYT} 
%\jay{Please cite SRAM/DRAM based NN accelerator work here} 
places logic in memory controllers
for volatile SRAM/DRAM memory modules.

%\jay{Please cite ReRAM or other NVM based NN accelerator work here. 
%\url{https://www.dropbox.com/s/0vx3kzudc1p9rch/make-01-00005.pdf?dl=0}} 
FPSA~\cite{FPSA}, and LerGAN~\cite{LerGAN}, Sparse ReRAM engine~\cite{SReRAME}, PRIME~\cite{PRIME}, PipeLayer~\cite{PipeLayer}, Zhang et al. ~\cite{EHECNP}
and FloatPIM~\cite{FloatPIM} 
leverage the fact that the physical 
characteristics of resistive random-access memory (ReRAM) technologies that
naturally implement a binary NN as the total current of each bitline
represents a result of multiplication and accumulation by carefully programming the resistance and 
conductance within cells and mapping inputs into supply voltage of each
wordline.

Though these accelerators have different
microarchitectures, all aforementioned hardware accelerators share the 
same spirit as \etpu{}s in the nature of using tensors/matrices as the basic
unit of processing. \GPTPU{} can easily adapt to any of these accelerators
as long as these accelerators expose their instruction set architectures
appropriately.

% Mention some sparse matrix NN accelerators.
This paper does not focus on sparse matrices as we have seen NN accelerators
that implicitly optimize for sparse matrices including SCNN~\cite{SCNN}, SparTen~\cite{SparTen}, Sparch~\cite{zhang2020sparch}, SIGMA~\cite{SIGMA}, Cambricon~\cite{Cambricon}, Bit-Tactical~\cite{Bit-Tactical},
OuterSPACE~\cite{OuterSPACE}, Laconic ~\cite{Laconic}, Bit Fusion~\cite{BitFusion} and Rhu, et al.~\cite{rhu2018compressing}
%\jay{Please add NN accelerators with hardware for sparse matrices}. 
This is even true for Nvidia's latest Ampere
architecture. With these accelerators automatically transform user inputs, 

 However, these architectures are currently not in
production. Commercially available ML accelerators, including Khadas VIM3, Rockchip
RK1808, Sophon BM1880, HiKey970, Jetson Nano, do not offer more competitive performance
and energy-efficiency than Edge TPUs. 

~\ignore{NGPUs~\cite{YazdanbakhshNGPU},
NPUs~\cite{EsmaeilzadehNPU}, GANAX~\cite{GANAX}, DianNao~\cite{DianNao},
Minerva~\cite{Minerva}, FA3C~\cite{FA3C}, Laconic~\cite{Laconic}, SCNN~\cite{SCNN}, Simba~\cite{Simba}, SparTen~\cite{SparTen}, eCNN~\cite{eCNN}, ExTensor~\cite{ExTensor}, Manna~\cite{Manna}, Diffy~\cite{Diffy}, HyGCN~\cite{HyGCN}, SIGMA~\cite{SIGMA}, PIXEL~\cite{PIXEL}, E-RNN~\cite{E-RNN}, VIP~\cite{VIP}}
~\ignore{valid list: 
V(1)HyGCN
V(2).  Automated Systolic Array Architecture Synthesis for
High Throughput CNN Inference on FPGAs (DAC,'17)
V(3)SCALE-Sim: Systolic CNN Accelerator Simulator (arXiv, '18)
V(4)Caffeine: Towards Uniformed Representation and Acceleration
for Deep Convolutional Neural Networks(ICCAD, '16)
X(5).  An OpenCL(TM) Deep Learning Accelerator on Arria 10(FPGA, '17)
V(6)Gemmini: An Agile Systolic Array Generator Enabling Systematic Evaluations of Deep-Learning Architectures (arXiv, '19)
X(*7) Eyeriss: An energy-efficient reconfigurable accelerator for deep convolutional neural networks. IEEE Journal of Solid-State Circuits 52, 1
(2017)
V(8)Chain-NN: An energy-efficient 1D chain architecture for accelerating deep convolutional neural networks. (DATE, '17). 
}



==> tableBenchmark.tex <==
\begin{table*}[t]
%\footnotesize
\scriptsize
%\small
\centering
%\hspace*{-0.2in}
\begin{tabular}{|l|l|c|c|c|l|l|}
\hline
			&  		    &
\multicolumn{2}{|c|}{\textbf{Dimensionality}} 		   &
\textbf{Data Size}& \textbf{Kernel Sub-}& \textbf{Source of} \\
\cline{3-4}
\textbf{Workload Name}	& \textbf{Category} & \textbf{Data} &
 \textbf{Kernel} & \textbf{(Elements)} & \textbf{dimension size} & \textbf{Baseline}\\
\hline
Breadth-First Search (BFS) & Graph Traversal & \multirow{2}{0.1in}{2D} & 1D &
\multirow{2}{0.55in}{65536\x{}65536} & 65536 & Rodinia~\cite{RodiniaBenchmark}\\ \cline{1-2}\cline{4-4}\cline{6-7}
Bellman-Ford (SSSP) & Graph Traversal & & 2D
 & & 65536\x{}4096 & Parallel Implementation of Bellman Ford Algorithm~\cite{bellmanford}\\ \hline
%CNN+LSTM~\cite{tensorflow2015-whitepaper} & Sentiment Classification & Sample & 25\% & 150~MB~\cite{Twitter}
%& < -0.01\% \\
Block-GEMM (GEMM) & Linear Algebra & \multirow{1}{0.1in}{2D} & 2D  &
65536\x{}65536 & 8192\x{}8192
&  MSplitGEMM with cuBLAS using Tensor Cores~\cite{MSplitGEMM,cuBLAS}\\ \hline
% High Correlation Analysis (HCA) & Statistics & 3D &
% 2D &	65536\x{}65536 & ~\cite{song2016canonical}\\ \hline
Hotspot (Hotspot) & Physics Simulation & 2D &
2D &	65536\x{}65536 & 4096\x{}4096 & Rodinia~\cite{RodiniaBenchmark,huang2006hotspot}\\ \cline{1-2}\cline{4-4}\cline{6-6} \hline
K-Means (KMeans) & Data Mining & \multirow{2}{0.1in}{2D} &
1D &	\multirow{2}{0.55in}{65536\x{}65536} & 65536 & Rodinia~\cite{RodiniaBenchmark}, Parallel K-Means Data Clustering~\cite{CPUkmeans, GPUkmeans}\\ \cline{1-2}\cline{4-4}\cline{6-7}
K-Nearest Neighbor  (KNN) & Data Mining &  &
1D &	 & 65536 & Rodinia~\cite{RodiniaBenchmark}, knn-CUDA~\cite{garcia2010k, knncuda}\\ \hline
PageRank  (PageRank) & Graph & \multirow{1}{0.1in}{2D} &
2D &	65536\x{}65536 & 4096\x{}65536 & GraphBlast~\cite{DBLP:journals/corr/abs-1908-01407}, GraphChi~\cite{kyrola2012graphchi}\\
\hline
%PageRank-Ext  (PageRank-Ext) & Graph &  &
%2D &	 & 4096\x{}65536 & GraphBlast~\cite{DBLP:journals/corr/abs-1908-01407}, GraphChi~\cite{kyrola2012graphchi}\\ \hline
2D Convolution (Conv2D) & Image Processing &
\multirow{1}{0.1in}{2D} &
2D &	65536\x{}65536 & 4096\x{}4096 & CUDA Separable Convolution~\cite{podlozhnyuk2007image}\\ \hline
Tensor Times Vector  (TTV) & Tensor Algebra & \multirow{2}{0.1in}{3D} &
2D/1D &	\multirow{2}{0.7in}{2048\x{}2048\x{}2048} & 512\x{}512 & NVIDIA~\cite{TensorContractions, ceckapro}\\ \cline{1-2}\cline{4-4}\cline{6-7}
Tensor Contractions  (TC) & Tensor Algebra & &
2D &	 & 512\x{}512 & NVIDIA~\cite{TensorContractions, ceckapro}\\ \hline
\end{tabular}
%\vspace{-2mm}
\vspace{+0.1in}
\caption{Workloads, the sources of their baseline implementations, the dimensionality, size of their raw data and the dimensionality
of their compute kernels.}
\label{table:benchmark}
% \vspace{-0.2in}
\end{table*}
%Text Generation& Generative model	& LSTM & Nietzsche's writings & 0.6~MB \\
%& Generative model	& LSTM & Nietzsche's writings & 0.6~MB \\
%Translation  	 & Neural Translation	& LSTM & Tatoeba & 10~MB \\
%CIFAR10-Resize    & Image Classification & CNN + Fully-connected & CIFAR10 & 163~MB \\
%PTB         & Language Modeling	& LSTM & PTB & 34~MB \\
%Abalone        & Classification based on Features & CNN & UCI Abalone dataset & 150~KB \\

